Regiones HII Gigantes en Galaxias Observables desde el Hemisferio Sur

In this thesis we presented a detailed spectroscopic study in a sample of Giant HII Regions in galaxies visible from Southern Hemisphere.

==> mem2.tex <==
\begin{minipage}{8cm}
\begin{picture}(0,0)
%\put(-20,-120)
%\put(-20,-150)
\put(200,-310)
{\special{psfile=firma-gb.eps hscale=100 vscale=100}}
\end{picture}
\vspace{1cm}
\end{minipage}


